Evolving Code with A Large Language Model

Algorithms that use Large Language Models (LLMs) to evolve code arrived on the Genetic Programming (GP) scene very recently. We present LLM GP, a formalized LLM-based evolutionary algorithm designed to evolve code. Like GP, it uses evolutionary operators, but its designs and implementations of those operators radically differ from GP's because they enlist an LLM, using prompting and the LLM's pre-trained pattern matching and sequence completion capability. We also present a demonstration-level variant of LLM GP and share its code. By addressing algorithms that range from the formal to hands-on, we cover design and LLM-usage considerations as well as the scientific challenges that arise when using an LLM for genetic programming.

==> figures/preliminary_sr_comparisons/results_table.tex <==
\begin{table}
\caption{Results for methods for Symbolic Regression. Average over 30 runs. Duration is run time. Cost is USD.}
\label{tab:results_main}
\begin{tabular}{lrrr}
\toprule
 & t & (t) & Cost \\
Name &  &  &  \\
\midrule
GP+LLM & 1664.30 & 1033.97 & NaN \\
GP+LLM M, Xo & 743.31 & 508.70 & NaN \\
PonyGP & 0.10 & 0.08 & NaN \\
Random & 0.18 & 0.01 & 0.00 \\
LLM & 837.16 & 416.12 & 2.63 \\
\bottomrule
\end{tabular}
\end{table}

